Bayesian Principles Improve Prompt Learning In Vision-Language Models

Prompt learning is a popular fine-tuning method for vision-language models due to its efficiency. It requires a small number of additional learnable parameters while significantly enhancing performance on target tasks. However, most existing methods suffer from overfitting to fine-tuning data, yielding poor generalizability. To address this, we propose a new training objective function based on a Bayesian learning principle to balance adaptability and generalizability. We derive a prior over the logits, where the mean function is parameterized by the pre-trained model, while the posterior corresponds to the fine-tuned model. This objective establishes a balance by allowing the fine-tuned model to adapt to downstream tasks while remaining close to the pre-trained model.

==> Manuscript/latex_for_20241005.tex <==
\section{Temporary section}

We now describe how we perform tractable posterior inference in our model with Gibbs sampling.
Define the matrix $\bm{A} \triangleq \text{OVE-MATRIX}(\bm{Y})$ to be a $CN \times CN$ sparse block matrix with $C$ row 
partitions and $C$ column partitions. Each block $\bm{A}_{cc'}$ is a diagonal $N \times N$ matrix defined as follows:
\begin{equation}
    \bm{A}_{cc'} \triangleq \text{diag}(\bm{Y}_{\cdot c'}) - \mathbb{1}[c = c'] \bm{I}_N,
\end{equation}
where $\bm{Y}_{\cdot c'}$ denotes the $c'$th column of $\bm{Y}$. Now the binary logit vector $\bm{\psi} \triangleq \bm{A} \bm{f} \in \mathbb{R}^{CN}$ will have entries equal to $f_{ci} - f_{c'i}$ for each unique combination of $c$ and $i$, of which there are $CN$ in total. The OVE composite likelihood can now be written as $\mathcal{L}(\bm{\psi} | \bm{Y}) = 2^N \prod_{j=1}^{NC} \sigma(\psi_j)$, where the $2^N$ term arises from the $N$ cases in which $\psi_j = 0$ due to comparing the ground truth logit with itself.

Analogous to (5), the likelihood of $\bm{\psi}$ conditioned on $\bm{\omega}$ and $\bm{Y}$ is proportional to a diagonal Gaussian:
\begin{equation}
    \mathcal{L}(\bm{\psi} | \bm{Y}, \bm{\omega}) \propto \prod_{j=1}^{NC} e^{-\omega_j \psi_j^2 / 2} \kappa_j^{\psi_j} \mathcal{N}(\bm{\Omega}^{-1/2} \bm{\kappa} | \bm{\psi}, \bm{\Omega}^{-1}),
\end{equation}
where $\kappa_j = 1/2$ and $\bm{\Omega} = \text{diag}(\bm{\omega})$. By exploiting the fact that $\bm{\psi} = \bm{A} \bm{f}$, we can express the likelihood in terms of $\bm{f}$ and write down the conditional composite posterior as follows:
\begin{equation}
    p(\bm{f} | \bm{X}, \bm{Y}, \bm{\omega}) \propto \mathcal{N}(\bm{\Omega}^{-1/2} \bm{\kappa} | \bm{A} \bm{f}, \bm{\Omega}^{-1}) \mathcal{N}(\bm{f} | \bm{\mu}, \bm{K}) \propto \mathcal{N}(\bm{f} | \bm{\Sigma}(\bm{K}^{-1} \bm{\mu} + \bm{A}^\top \bm{\kappa}), \bm{\Sigma}),
\end{equation}
where $\bm{\Sigma} \triangleq (\bm{K}^{-1} + \bm{A}^\top \bm{\Omega} \bm{A})^{-1}$, which is an expression remarkably similar to (6). Analogous to (7), the conditional distribution over $\bm{\omega}$ given $\bm{f}$ and the data becomes $p(\bm{\omega} | \bm{f}) = \text{PG}(\bm{\omega} | 1, \bm{A} \bm{f})$.

==> notations.tex <==
\newcommand{\punt}[1]{}

\usepackage{amsthm}
% \usepackage{xcolor}
\usepackage{hyperref}

\usepackage[dvipsnames]{xcolor}
\usepackage{microtype}
\usepackage{lmodern}
\usepackage[T1]{fontenc}

\newcommand{\inv}{^{-1}}
\newcommand{\trp}{{^\top}} % transpose
\newcommand{\onehlf}{\frac{1}{2}}
\newcommand{\tonehlf}{\tfrac{1}{2}}
\renewcommand{\eqref}[1]{eq.~\ref{eq:#1}}
\newcommand{\Nrm}{\mathcal{N}}
% \newcommand{\Tr}{\mathrm{Tr}}
% \newcommand{\diag}{\mathrm{diag}}
%\DeclareMathOperator*{\argmin}{arg\,min}
%\DeclareMathOperator*{\argmax}{arg\,max}
% \newcommand{\figref}[1]{Fig.~\ref{fig:#1}}  % use for citing figs
% \newcommand{\secref}[1]{Sec.~\ref{sec:#1}}
\newcommand{\subsecref}[1]{Subsec.~\ref{subsec:#1}} % use for citing secs
\newcommand{\tabref}[1]{Table ~\ref{tab:#1}}  % use for citing tables
\newcommand{\algoref}[1]{Algorithm~\ref{algo:#1}}  % use for citing algorithms
% \newcommand{\propref}[1]{Prop.~\ref{prop:#1}}
\newcommand{\rmrkref}[1]{Remark.~\ref{rmrk:#1}}
\newcommand{\lemmaref}[1]{Lemma.~\ref{lemma:#1}}
% \newcommand{\defnref}[1]{Defn.~\ref{defn:#1}}
% \newcommand{\thmref}[1]{Thm.~\ref{thm:#1}}
\newcommand{\suppsecref}[1]{Supplementary Sec.~\ref{supp:#1}}  

% ----- Math definitions -------------------
% \newcommand{\vx}{\mathbf{x}}
% \newcommand{\vu}{\mathbf{u}}
\newcommand{\var}{\mathrm{var}}
\newcommand{\Dat}{\mathcal{D}}

\newcommand{\Ev}{\mathcal{E}}
\newcommand{\vxloc}{\mathcal{X}}
\newcommand{\vkx}{\mathbf{k_x}}
% \newcommand{\vv}{\mathbf{v}}
\newcommand{\vky}{\mathbf{k_y}}
% \newcommand{\vf}{\mathbf{f}}
% \newcommand{\vb}{\mathbf{b}}
\newcommand{\valpha}{\mathbf{\ensuremath{\bm{\alpha}}}}
\newcommand{\vbeta}{\mathbf{\ensuremath{\bm{\beta}}}}
\newcommand{\vphi}{\mathbf{\ensuremath{\bm{\phi}}}}
\newcommand{\vpsi}{\mathbf{\ensuremath{\bm{\psi}}}}
\newcommand{\bmu}{\mathbf{\ensuremath{\bm{\mu}}}}
% \newcommand{\vu}{\mathbf{u}}
% \newcommand{\vk}{\mathbf{k}}
\newcommand{\bK}{\mathbf{K}}
%\newcommand{\E}{\mathbb{E}}
\newcommand{\Vm}{\mathbb{V}} 
% \newcommand{\vone}{\mathbf{1}} % one vector
% \newcommand{\vm}{\mathbf{m}}
% \newcommand{\vz}{\mathbf{z}}
% \newcommand{\vw}{\mathbf{w}}
% \newcommand{\vr}{\mathbf{r}} 
% \newcommand{\vs}{\mathbf{s}} 
% \newcommand{\ve}{\mathbf{e}} 
% \newcommand{\vd}{\mathbf{d}} 
\newcommand{\fmap}{\bm{\lambda}{_{map}}}
\newcommand{\bphi}{\bm{\phi}}
\newcommand{\phimap}{{\hat {\bm{\phi}}}{_{map}}}
\newcommand{\fmapstar}{\mathbf{f^*_{map}}}
\newcommand{\muf}{\ensuremath{\mu_f}}
\newcommand{\vmuf}{\mathbf{\ensuremath{\bm{\mu}_f}}}
\newcommand{\vpi}{\mathbf{\ensuremath{\bm{\pi}}}}
% \newcommand{\vmu}{\mathbf{\ensuremath{\bm{\mu}}}}
% \newcommand{\vtheta}{\mathbf{\ensuremath{\bm{\theta}}}}
\newcommand{\LL}{\ensuremath{\mathcal{L}}}
\newcommand{\vlam}{\bm{\lambda}}
% \newcommand{\mR}{\mathbf{R}}
% \newcommand{\mW}{\mathbf{W}}
% \newcommand{\mZ}{\mathbf{Z}}
% \newcommand{\mC}{\mathbf{C}}
% \newcommand{\mX}{\mathbf{X}}
% \newcommand{\mI}{\mathbf{I}}
% \newcommand{\mK}{\mathbf{K}}
% \newcommand{\mA}{\mathbf{A}}
% \newcommand{\mY}{\mathbf{Y}}
\newcommand{\vX}{\mathcal{X}}
\newcommand{\vK}{\mathbf{K}}
% \newcommand{\mJ}{\mathbf{J}}
% \newcommand{\vn}{\mathbf{n}}
%\renewcommand{\RR}

\newcommand{\Em}{\mathbb{E}}
% \newcommand{\Vm}{\mathbb{V}}

% \newcommand{\set}[1]{\{#1\}}
\newcommand{\kml}{{\hat \vk}_{ML}}
% \newcommand{\vy}{\mathbf{y}}
% \newcommand{\vc}{\mathbf{c}}
% \newcommand{\vh}{\mathbf{h}}
% \newcommand{\vp}{\mathbf{p}}
% \newcommand{\vt}{\mathbf{t}}
% \newcommand{\vg}{\mathbf{g}}
\newcommand{\Lprior}{\Lambda_p}
\newcommand{\Lix}{L_{x}}
\newcommand{\thetmap}{\theta_{\mu}}
\newcommand{\Lmap}{\Lambda_\mu}
\newcommand{\thetli}{\theta_{l}}
\newcommand{\Lli}{\Lambda_{l}}
\newcommand{\nsevar}{\sigma^2}
\newcommand{\nsestd}{\sigma}
\newcommand{\vchi}{\bm{\chi}}
\newcommand{\vomega}{\bm{\omega}}
% \newcommand{\tr}{^\top}
% \newcommand{\vphi}{\mathbf{\ensuremath{\bm{\phi}}}}
\newcommand{\vtau}{\mathbf{\ensuremath{\bm{\tau}}}}
\newcommand{\vkappa}{\mathbf{\ensuremath{\bm{\kappa}}}}

\newtheorem{thm}{Theorem}[section]
\newtheorem{lem}{Lemma}[section]
%\newtheorem{claim}[thm]{Claim}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{prop}[thm]{Proposition}
% \newtheorem{prop}{Proposition}
% \newtheorem{remark}{Remark}
\newtheorem{defn}{Definition}[section]
%\theoremstyle{definition}
\newtheorem{condition}{Condition}
% \newtheorem{thm}{Theorem}[section]
\def\argmax{\mathop{\rm arg\,max}}
\def\argmin{\mathop{\rm arg\,min}}

\def\Pr{\ensuremath{\text{Pr}}}
% Definition





==> src/tab_generalization.tex <==
% \begin{table}[t]
% \centering
% \resizebox{1.0\columnwidth}{!}{
% \begin{tabular}{l|l|cc|cc}
% \toprule[0.15em]
%  & & \multicolumn{2}{c|}{CoOp} & \multicolumn{2}{c}{CoCoOp} \\
%  & & SoftMax & OVE-PG & SoftMax & OVE-PG \\
% \midrule
% \textbf{Source} & ImageNet & xx.xx & xx.xx & xx.xx & xx.xx  \\ \midrule
% \multirow{4}{*}{\textbf{Target}} & ImageNet-V2 & xx.xx & xx.xx & xx.xx & xx.xx \\
%  & ImageNet-S & xx.xx & xx.xx & xx.xx & xx.xx \\
%  & ImageNet-A & xx.xx & xx.xx & xx.xx & xx.xx  \\
%  & ImageNet-R & xx.xx & xx.xx & xx.xx & xx.xx  \\
%  \midrule
%  \multicolumn{2}{c|}{\textit{Average}} & xx.xx & xx.xx & xx.xx & xx.xx \\
% \bottomrule[0.12em]
% \end{tabular}
% }
% \caption{Comparison of accuracy (\%) on cross-dataset performance between Softmax and OVE-PG (Ours) for CoOP and CoCoOp. The best performance within each shared base algorithm is highlighted in \textbf{bold}.}
% \label{table:generalization}
% \end{table}
